DeepLight: Robust & Unobtrusive Real-time Screen-Camera Communication for Real-World Displays

The paper introduces a novel, holistic approach for robust Screen-Camera Communication (SCC), where video content on a screen is visually encoded in a human-imperceptible fashion and decoded by a camera capturing images of such screen content. We first show that state-of-the-art SCC techniques have two key limitations for in-the-wild deployment: (a) the decoding accuracy drops rapidly under even modest screen extraction errors from the captured images, and (b) they generate perceptible flickers on common refresh rate screens even with minimal modulation of pixel intensity. To overcome these challenges, we introduce DeepLight, a system that incorporates machine learning (ML) models in the decoding pipeline to achieve humanly-imperceptible, moderately high SCC rates under diverse real-world conditions. Deep-Light's key innovation is the design of a Deep Neural Network (DNN) based decoder that collectively decodes all the bits spatially encoded in a display frame, without attempting to precisely isolate the pixels associated with each encoded bit. In addition, DeepLight supports imperceptible encoding by selectively modulating the intensity of only the Blue channel, and provides reasonably accurate screen extraction (IoU values >= 83%) by using state-of-the-art object detection DNN pipelines. We show that a fully functional DeepLight system is able to robustly achieve high decoding accuracy (frame error rate < 0.2) and moderately-high data goodput (>=0.95Kbps) using a human-held smartphone camera, even over larger screen-camera distances (approx =2m).

==> algodraft.tex <==
\begin{algorithm}[t]
    \caption{Decoder frame synchronization algorithm}
    \label{alg:algo1}
    \begin{algorithmic}[1]
    \STATE $[frm_2,frm_1,frm] \leftarrow [nextFr(),nextFr(),nextFr()]$
    % \STATE $frame_1 \leftarrow  nextFrame()$
    % \STATE $frame \leftarrow  nextFrame()$
    \STATE $num_{seq} = -1$
    \WHILE {$frm != null$  (More frames present)}
        \STATE $screen\_position \leftarrow  ScreenExtract(frm)$
        \STATE $frm\_stack \leftarrow  stack(frm_2.B, frm_1.B, frm.B)$
        \STATE $screen\_extract \leftarrow  extract(frm\_stack, screen\_position)$ 
        \STATE $dnn\_data \leftarrow  DeepLight\_Decode(screen\_extract)$
        \STATE $error, rs\_data \leftarrow  RSDecode(dnn\_data)$
        \IF {$error == nil$}
            \IF {$csumPass(rs\_data)$}
                % \STATE $num_{seq} \leftarrow  rs\_data.seq\_num$
                \IF {$num_{seq} \in \{-1,(rs\_data.seq-1)\mod32$\}}
                    \STATE $data \leftarrow  rs\_data.getData()$;  
                    \STATE $num_{seq} \leftarrow  rs\_data.seq$
                    \STATE $seq\_time \leftarrow  frame.timestamp$
                \ELSE
                    \STATE $interval \leftarrow  frame.timestamp - seq\_time$
                    \STATE $inc \leftarrow  (rs\_data.seq - num_{seq})\textrm{ }mod\textrm{ }32$
                    \IF {$interval > \frac{2}{F_d} \times inc$ (sufficiently apart)}
                        \STATE $data \leftarrow  rs\_data.getData()$
                        \STATE $num_{seq} \leftarrow  rs\_data.seq$
                        \STATE $seq\_time \leftarrow  frame.timestamp$
                    \ENDIF
                \ENDIF
            \ENDIF
        \ENDIF
        % \STATE $frame_2 \leftarrow  frame_1$
        % \STATE $frame_1 \leftarrow  frame$
        \STATE $[frm,frm_1,frm_2] \leftarrow [nextFr(),frm,frm_1]$
    \ENDWHILE
    \end{algorithmic}
\end{algorithm}


==> misc.tex <==
Abstract
%original abstract moved outside by Archan
%The rapid growth of camera-embedded personal devices, together with the widespread deployment of digital displays, opens up opportunities for new forms of vision-driven, human-computer interactions. This paper tackles the problem of screen camera communication (SCC), whereby displays embed information (in a humanly imperceptible fashion) in their screen content, which is then decoded by the camera sensor. We show that state-of-the-art SCC techniques are not robust enough for practical, real-world use as their performance degrades significantly when confronted with several real-world shortcomings in the decoding pipeline--such as the inability to precisely delineate the screen boundaries or filter out captured images that have spurious coded information. Inspired by the recent success of DNNs in tackling vision problems, we then develop \names, an approach that overcomes these shortcomings via application of multiple, specialized DNN pipelines. Experimental evaluations show that this DNN-based approach indeed presents a simpler and robust solution, providing improved throughput while ensuring that the information remains visually imperceptible. More precisely, \am{have to include a line on key results.}


Intro:
%In addition, we shall describe, and practically demonstrate, how system-level design choices, such as the use of appropriate Reed-Solomon (RS) block code~\cite{XXX}, help achieve both identification/elimination of transition frames and moderately high \emph{goodput}, even under the real-world impairments and artefacts outlined above.

%each of which learns the salient latent features from a diverse set of labeled training \gj{datasets is more suitable than images}images. Our choice of ML-based mechanisms is motivated by the recent dramatic successes reported in the application of Deep Neural Network (DNN) models to various vision-based problems, including object detection and object localization, \emph{especially in the presence of noise}. More specifically, \name utilizes distinct DNN pipelines to address different challenges including: (a) Accurate Display Screen Detection—this is performed by using a modified object-detection DNN, which learns and exploits the pixel intensity variations that are characteristic of screen content; (b) Accurate Inference of Non-Transition Frames—this is performed by a modified LSTM-like DNN that takes multiple consecutive camera images as input and determines the best representative non-transition images, without any knowledge of the underlying frame rate or without needing explicit embedded markers; and (c) Accurate Bit Decoding without Perfect Spatial Alignment—-this is performed by a low-complexity Convolutional DNN that to recover individual code bits without being explicitly aware of the grid of pixels corresponding to each bit.  Besides describing each of these individual components, we shall provide a real-world empirical evaluation of the robust operational of the overall \name system.

%Overall, \name is notable for being the first to propose a deep learning-based approach for decoding and demonstrate its superiority, over prior signal processing-based approaches, under real world noise and impairments, for SCC.

\iffalse
\aash{if space permits}
The rest of the sections are organized as follows: Sec~\ref{sec:}-Design goals; Sec~\ref{sec:background}-Related work;Sec~\ref{sec:}-Limitations of existing SCC techniques;Sec~\ref{sec:}-\names overview;Sec~\ref{sec:}-\names ML based decoder;Sec~\ref{sec:}-Prototype implementation;Sec~\ref{sec:}-Evaluation;Sec~\ref{sec:}-Discussion;Sec~\ref{sec:}-Conclusion.
\fi

\iffalse 
\aash{I commented this out as I felt it seemed repetitive.}
We emphasize again that \name is a system that leverages on the core encoding mechanisms of prior SCC technologies such as HiLight~\cite{li2015real} and ChromaCode~\cite{zhang2019chromacode}. \name is notable for being the \emph{first to propose a deep learning-based approach for decoding and demonstrate its superiority, over prior signal processing-based approaches, under real world noise and impairments}.
\fi
%demonstrate

%selectively introducing DNN pipelines into the decoding process, and for demonstrating that such DNN-based approaches are more robust than pure signal processing-based approaches under real world noise and impairments.



---
Decoder


\iffalse
As mentioned previously, the core of our innovation is in the design of a deep neural network (DNN)-based robust decoder that employs ML techniques to collectively decode all the transmitted bits in a frame without explicitly requiring the precise extraction of pixels associated with each encoded bit/cell. In particular, we designed a Convolutional Neural-Network (CNN) model that can extract the subtle temporal variation of Blue channel intensity across each individual cell, where each cell consists of a collection of a subset (e.g., $9 \times 9$) pixels. Figure~\ref{fig:cnn_model_features}a) shows the structure of our proposed CNN model , whereas ~\ref{fig:cnn_model_features}(b) visually illustrates the extracted features at layer 2 of this CNN. Our choice of a CNN-based approach is motivated by the remarkable capability shown by CNNs to perform the spatial filtering and reasoning needed to execute several complex vision tasks (such as object detection~\cite{XXX}, image classification and visual question answering) with near-human accuracy, even under complex/cluttered conditions. 

\begin{figure}
	\centering
	\includegraphics[width=\linewidth]{figures/cnn_model_features.pdf}
	\caption{The \name CNN Decoder Model.}
	\label{fig:cnn_model_features}
\end{figure}

The input to our CNN model is an image with $L=3$ channels, with each channel corresponding to the pixel value of the Blue Channel of $L$ consecutive frames. These $L$ frames effectively capture both the rising (F+) and falling (F-) sequence of Manchester coded images. ($L=3$ is used simply as an exemplar to illustrate our logic and is based on the assumption that the camera sampling rate is twice the display frame rate, as minimally required by the Nyquist criterion. In Section~\ref{sec:XXX}, we shall elaborate on how the approach can be generalized with larger values of $L$, to support decoding without any explicit knowledge of the display frame rate.) The first layers is a $1 \times 1$ convolutional layer, that is used to extract different \emph{temporal} relationships, for each pixel, across the $L=3$ consecutive frames. The model then includes several additional  convolutional layers that extract higher-level and multi-scale features in the input data,  corresponding to a hybrid mix of spatial (across the neighboring pixels of a single image) and temporal (across the corresponding pixels of multiple frames) features at different levels of granularity. A finally fully-connected layer, with a Sigmoidal activation function, is used to regress the value of each bit, such that the final output of the CNN is a vector of $M\times N$ bits. We emphasize this key property: \textbf{each of the final $M\times N$ bits of output is derived from the holistic processing of $L$ \emph{entire} frames, rather than via an isolated processing of a predesignated subset of pixels.}  It is this holistic processing that provides \name the robustness that we desire, enabling it extract the entire set of encoded bits via collective analysis of variations across the entire image. 
\fi

evaluation

\iffalse   
    \item \emph{Throughput} ($GP$), defined as the total number of bits, per second, effectively (correctly) decoded by the \name decoder. $T$ is computed as: 
    \begin{equation}
        T = (D + Seq + Csum + RS) \times Fr \times (1-FER)
    \end{equation}
        Where $D$ is the number of data bits/frame,  $Seq$ is the number of bits used for the sequence number, $Csum$ is the number of checksum bits, $RS$ is the number of error-correction bits, $Fr$ is the data frame rate (for Manchester encoding, this is half of display rate), and $FER$ is the frame error rate--i.e., the fraction of data frames that are correctly decoded, after Reed-Solomon error correction.   
\fi


% \begin{figure}
% \begin{minipage}{0.49\linewidth}
%     \centering
% 	\includegraphics[height=1.3in,width=\textwidth]{figures/perf_vs_distance_delta_fer.pdf}
% 	%\caption{\names: FER for different (D,$\Delta$).}
% 	%\label{fig:perf_delta}
% \end{minipage}
% \hfill
% \begin{minipage}{0.49\linewidth}
%     \centering
% 	\includegraphics[height=1.3in,width=\textwidth]{figures/perf_vs_distance_delta_gp.pdf}
% 	%\caption{\names: GP for different (D,$\Delta$).}
% 	%\label{fig:perf_delta}
% \end{minipage}
%  \label{fig:perf_delta}
% \caption{\names: FER/GP for different (D, $\Delta$).}
% \end{figure}

Discussion
%The bit errors are assumed to be random throughout this study. But further analysis showed several trends/patterns when it come to the probability of a bit error occurring. The encoded bit pattern can increase/decrease the probability. When it comes to the 16 possible bit configurations in a $2 \times 2$ bit block on the screen, the probability is the highest when all bits are zeros or ones. This trend holds for larger blocks as well. 



\iffalse
\aash{I embedded this in Introduction section}
Before proceeding to an in-depth description of \names, we first describe a canonical use case for practical SCC using personal mobile devices in public spaces, and thereby derive some of the features desired of a useful solution.

\begin{figure}
	\centering
	\includegraphics[width=\columnwidth,height=2.1in]{figures/usecase.jpg}
	\caption{Practical, Multi-User, Multi-Display SCC using Mobile/Wearable Devices}
	\label{fig:scc-usecase}
\end{figure}

\noindent \textbf{Visible Light Audio \& Text Transmission:} We envisage a scenario, such as an airline lounge, where SCC is used to transmit and encode a stream of supplementary information that accompanies the primary video content being displayed on multiple public displays. As shown in Figure~\ref{fig:scc-usecase}, two different users U1 and U2 are viewing two separate displays, one carrying a live feed of a sporting event while the other carries an update of flight-related information. Given the presence of multiple passengers, possibly with different language preferences, in this quiet area, the audio feeds of both streams are muted. However, SCC is used to visually and subliminally encode the following supplementary information: (a) for the live viewing of sports, SCC is used to transmit the audio channel containing the sports commentary; (b) for the flight information display, SCC transmits structured textual information (in multiple languages) describing various alerts and the status of various flight schedules. User U1 watches the sports feed with a see-through head-mounted, camera-equipped display (e.g., a pair of glasses with a clip-on camera): the \name software running on the camera is able to decode the sports commentary, in real time, and then output this via a personal speaker (e.g., Bluetooth-enabled earphones). On the other hand, user U2 point her camera-equipped smartphone at the flight information display: the \name software running on her smartphone is able to decode the visually-encoded multi-lingual text commentary and then overlay the information in U2’s native/preferred language (configured as a static profile parameter) on her smartphone. It is pertinent to note that: (a) the audio or textual information is transmitted only via visual encoding of the screen content—there is no secondary wireless transmission (e.g., via WiFi or Bluetooth) of this content, and users are not required to perform any additional action, such as `configuring’ or connecting their devices to specific wireless channels; (b) the user’s reception of such SCC information is not only seamless but \emph{attention-driven}—i.e., supplemental information is only decodable if the user’s personal device actually points to and captures the corresponding display, and the audio stream is automatically terminated as soon as user U1 looks away from the sports screen; and (c) the scenario is completely non-intrusive, with other non-\name users in the lounge being completely unaware of the transmission of any such supplementary information.
\fi

Evaluation
\iffalse
\noindent{\bf Supplement materials for reference:} We have provided a demo video of \name end-end performance and access to our flicker perception experiment videos and protocol here:\url{}.
\fi


%istance (1m50). 5 out of 7 users even still achieve a FER $\le 0.2$ at 1m75 (GP $\ge 0.95kbps$). The FER of user P3 at 1m00 is lower than 1m50 and 1m75. This is not because some areas in the video content have a color similar to the background. At shorter distance, the screen appears larger in the camera frame and the screen extractor is confused and lose a large part of the screen. User P7 hands were too shaky compared to other users. Strong vibrations make pixels blurry, and the value of each pixel is a mixture of many neighboring pixels. We believe it is the reason the FER of \names on P7 is considerably higher. The results show that \names~ can tolerate normal hand motion artifacts.

%\subsubsection{Discussion}
%We make the following observations from our evaluation:

%-- MOS for our system is as good as for the original, unmodified video. 

%-- MOS for Chromacode is close to average implying users still feel the flicker is perceptible. 

%-- The PSNR variation among the compared methods ...


%In this section, we evaluate the end-to-end \names~ system with users. We shows different short videos embedded with ramdom data on a desktop monitor (the same videos and screen we used for micro-benchmarks). We asked 7 different users to hold a camera (iPhone X) to record the screen. Each user was asked to sit on a chair at different distances including 1m15, 1m65, 1m90 and 2m15. As the users stretch their arm forward when pointing the camera toward the screen, the actual distance from the camera to the screen is $\approx 0m9, 1m40, 1m65 and 1m90$. We explicitly asked the users \emph{not} to rely their elbow on the chair arms as it suppresses most of the hand movements. Each user recorded 10 different short videos. In this experiment, we use our \names~screen extractor to extract the screen. 

